Adversarial Black-Box Attacks on Automatic Speech Recognition Systems using Multi-Objective Evolutionary Optimization

Fooling deep neural networks with adversarial input have exposed a significant vulnerability in the current state-of-the-art systems in multiple domains. Both black-box and white-box approaches have been used to either replicate the model itself or to craft examples which cause the model to fail. In this work, we propose a framework which uses multi-objective evolutionary optimization to perform both targeted and un-targeted black-box attacks on Automatic Speech Recognition (ASR) systems. We apply this framework on two ASR systems: Deepspeech and Kaldi-ASR, which increases the Word Error Rates (WER) of these systems by upto 980%, indicating the potency of our approach. During both un-targeted and targeted attacks, the adversarial samples maintain a high acoustic similarity of 0.98 and 0.97 with the original audio.

==> approach.tex <==

\section{Approach}

We propose a framework to generate adversarial samples based on the principles of multi-objective evolutionary algorithms (MOEA). This framework is demonstrated in Fig. 2. A genetic algorithm(GA) maintains a population of solutions(individuals) and implements a survival-of-the-fittest strategy for exploring best-fitting solutions. The common scheme of any MOEA in- cludes the same steps as any conventional one-criterion GA, but in contrast to it, the outcome of a MOEA is the set of non- dominated points which form the Pareto set approximation[]. This problem can be formulated as:
Eqn.~\ref{eqn:1}, where $N$ is the number of objective criteria :
\begin{equation}
    \forall i \epsilon \{1,..,N\}  \min\diagup\max f_{i}(\vec{x})
    \label{eqn:1}
\end{equation}

The aim is to determine  a set of $\vec{x}^{*}$ which yields the optimum value of all the functions. In our system, $\vec{x}$ denotes the audio sample.  A candidate solution $\vec{x_i}$ is said to dominate another solution $\vec{x_j}$, if $\vec{x_i}$ is no worse than $\vec{x_j}$ in all objectives and $\vec{x_i}$ is strictly better than $\vec{x_j}$ in at least one objective. Multi-objective schemes with conflicting objective functions often give rise to a set of two or more optimal solutions because none of them can be considered as better than the other(s) concerning all objective functions. These optimal solutions are known as \textit{Pareto-optimal} solutions \cite{pareto}. %For designing a MOGA, some issues faced are fitness assignment strategies, diversity preservation techniques, and ways of elitism implementation.

In our framework we propose to use two objectives to calculate each individual's fitness score: i) the Euclidean distance between the \textit{Mel-frequency cepstral coefficients} (MFCC) \cite{mfcc} of the original and the generated audio samples, and ii) the \textit{edit distance} between the texts generated by the ASR system when the original and generated sample are provided as inputs. Approaches  like \cite{Alzantot_bb} use the score of the model and \cite{Rohan_BB} use text similarity as a single criterion to generate adversarial sample. These works have ignored acoustic similarity, which is a strong indicator of the goodness of an individual. An audio sample is considered to be a good adversary, if it sounds very similar to the original sample but generates an entirely different text. Hence the sample generated should have: i) maximum acoustic similarity and minimum text similarity (for un-targeted attacks), or ii) maximum acoustic similarity and maximum text similarity with a target text (for targeted attacks). We achieve this by introducing a fitness function with multiple objectives which tries to strike a balance between acoustic and text similarities. 

The framework performs exploration of new individuals to add diversity to the solution space. This done by using carefully designed genetic operators for audio adversarial generation: 

\textbf{Crossover} This is applied on two individual identified as parents to generate a new offspring.  We use arithmetic recombination operators to perform a single-point crossover \cite{gen_algo}.If $(p_1, p_2)$ is a mating pair, then the three children are created to have the characteristics of the parents in equal proportion, and dominated by a particular parent. 
\begin{equation}
  \begin{gathered}
   C_{1}=\frac{p_{1}+p_{2}}{2}\\
   C_{2}=\frac{2 \times p_{1}+p_{2}}{3}\\
   C_{3}=\frac{ p_{1}+2 \times p_{2}}{3}
   \end{gathered}
\end{equation}

\textbf{Mutation} Once the off-springs are created, we mutate parts of their genes so that the new population becomes diverse and can hence be scattered over a larger area in the search space by adding Gaussian noise to the genes with a probability $prob_m$. 
\textbf{We should highlight addition of Gaussian noise, how is it high frequency but goes unheard to human-- speech conference} 

Another important element in multi-objective evolutionary  algorithms is the Pareto front estimation. These algorithms comprise of different ranking schemes that alter the "fitness landscape" of the search space and accomplish fitness assignment, selection and maintain diversity to achieve a well-distributed Pareto Front. 

The ranking scheme proposed by Fonseca and Fleming [6] involved assigning an individual’s rank (in the objective function space) equal to the number of population individuals that dominated that individual; that is, the ranking was done according to the degree of domination; the more members of the current population that dominate a particular individual, the lower its rank. It, therefore, uses fitness sharing in the objective function space and mating is also restricted.  Our framework incorporates this ranking scheme as one the approaches. However, to suit our task at hand we modify the selection strategy.  We use an ensemble of techniques to create a diverse mating pool which is more likely to produce fitter individuals/adversarial samples:

 \begin{enumerate}
     \item \textit{Same Rank Selection}: In this selection scheme, we first create two lists $l_1$ and $l_2$ by ranking the individuals based on each of the two objectives. Let $l_x \gets i_{xr}$ where $i$ is an individual in list $x$ with rank $r$. We pair two $`i'$s which have the same $r$ in the two lists. 
    \item \textit{Inverse Rank Selection}: This scheme is the opposite of the previous one. One list is ranked from best to worst and the other vice-versa. This makes sure that diversity is maintained in the population and we do not constraint the search space.
    \item \textit{Roulette Wheel Selection} \cite{roulettewheel}:
     In this scheme, the fitness score is used to compute a probability of selection for each individual. If $f_{i}$ is an individual $i$'s fitness score, then its probability of being selected is: 
     \begin{equation}
         p_{i}=\frac{f_{i}}{\sum_{i=1}^N f_{i}}
     \end{equation}
     where $N$ is the number of individuals in the population. While unlikely, individuals with high fitness scores may still be eliminated ensuring there is no premature convergence to local optima.
 \end{enumerate}

The main strength of MOGA is that it is efficient and relatively easy to implement. It has also been successful in solving optimal control problems where it has exhibited very good overall performance [32].
%Reproduction probabilities were determined by means of exponential ranking. Afterwards the fitness values were averaged and shared among individuals having identical ranks [15]. Finally, stochastic universal sampling, which provides zero bias and minimum spread (i.e., the range of possible values for the number of offspring of an individual) was used to fill the sampling pool.


Another successful technique is NSGA-II\cite{}.  Pareto front is obtained using non-dominated sorting.  This sorting ranks individuals by iteratively determining the nondominated solutions in the population, assigning those individuals the next best  hrank and removing them from the population.
%Consequently Deb et al. [34] developed a second-generation algorithm, NSGA II. Convergence to the Pareto front is made possible by nondominated sorting. This sorting ranks individuals by iteratively determining the nondominated solutions in the population, assigning those individuals the next best rank and removing them from the population.

Favouring individuals with large crowding distances maintain diversity within one rank. After evaluating the offspring’s fitness (nondominated rank and crowding distance), parents and offspring fight for survival as Pareto dominance is applied to the combined population of parents and offspring. Then, the least dominated  solutions survive to make the population of the next generation. The sampling pool is filled using the tournament selection process, where a number of individuals (ranging from 2 to ) are chosen randomly and the “best” individual from that group is selected as parent for the next generation

%NSGA-II, being elitist, keeps as many nondominated solutions as possible, up to the size of the population [7]. The elitist selection is as follows. After evaluating the offspring’s fitness (nondominated rank and crowding distance), parents and offspring fight for survival as Pareto dominance is applied to the combined population of parents and offspring. Then, the least dominated  solutions survive to make the population of the next generation. The sampling pool is filled using the tournament selection process, where a number of individuals (ranging from 2 to ) are chosen randomly and the “best” individual from that group is selected as parent for the next generation
%Many approaches are now in use for MOEA (with different ranking schemes that alter the “fitness landscape” of the search space by adding more “ordering information”), and the key to their success lies in how they accomplish fitness assignment and selection and how they maintain diversity to achieve a well-distributed Pareto (trade-off) front 

%ranking of the population individuals.  This is done to obtain probabilities of survival and  are essential for the selection process.  Researchers have proposed multiple several techniques \cite{}.  Our framework to generate adversarial samples incorporates \textbf{Multi-objective genetic algorithm(MOGA)} \cite{} and
%\textbf{NSGA-2} \cite{}. In \cite{moga} individual’s rank corresponds to the number of
%individuals in the current population by which it is dominated.  


%\textbf{}

%In the proposed  framework the fitness function is computed on a potential solution (Individual). A set of solutions, comprising population undergoes the process of selection, crossover and mutation to generate new off springs  iteratively to form pareto set.   We propose the following techniques to perform each process: 

%\textbf{Mating Pool Identification (Selection):} This procedure created pairs of individuals which acts as parents to the next generation. Traditionally, this is done by picking the top-$k$ individuals with the best fitness scores and pairing them randomly. However, this does not work well when the fitness function has more than one objective to optimise. Therefore, we use an ensemble of techniques to create a diverse mating pool which is more likely to produce fitter individuals to be potential adversarial samples:

% \begin{enumerate}
%     \item \textit{Same Rank Selection}: In this selection scheme, we first create two lists $l_1$ and $l_2$ by ranking the individuals based on each of the two objectives. Let $l_x \gets i_{xr}$ where $i$ is an individual in list $x$ with rank $r$. We pair two $`i'$s which have the same $r$ in the two lists. 
%     \item \textit{Inverse Rank Selection}: This scheme is the opposite of the previous one. One list is ranked from best to worst and the other vice-versa. This makes sure that diversity is maintained in the population and we do not constraint the search space.
%     \item \textit{Roulette Wheel Selection} \cite{roulettewheel}:
%     In this scheme, the fitness score is used to compute a probability of selection for each individual. If $f_{i}$ is an individual $i$'s fitness score, then its probability of being selected is: 
%     \begin{equation}
%         p_{i}=\frac{f_{i}}{\sum_{i=1}^N f_{i}}
%     \end{equation}
%     where $N$ is the number of individuals in the population. While unlikely, individuals with high fitness scores may still be eliminated ensuring there is no premature convergence to local optima.
% \end{enumerate}
 



% In the genetic systems, the fitness function is computed on a potential solution 
% In genetic systems, each potential solution is termed as an \textit{Individual}. Each individual's characteristics are determined by it's \textit{Genes}. %Genes can be thought of as analogous to model parameters. 
% The group of individual solutions in a genetic system is called its \textit{Population}. The population iteratively gets fitter over time resulting in more optimal solutions. The population in each iteration is known as a \textit{Generation}\footnote{Henceforth; we use the terms population and generation interchangeably}.
% At the beginning of the first generation, genes of the population are either randomly initialized or initialized according to some heuristics which helps the process to converge quickly.




% Outline of Proposed Approach: 
% 1. what is GA -3 lines
% 2. What is Multiobjective GA -- 3 lines
% 3. Why MOGA is important for adversarial generation problem, why use of acoustic similarity is important for ASR tasks comparision with single GA work  
% 4. Components to framework 
%     population
%     fitness computation
%     mating pool identification
%     crossover
%     mutation
%     Dominannce Evaluation
    
% 5. To generalise design of fitness function, mutation operation and crossover, we also evaluate NSGA2
% 6. NSGA2-- what is it and reference, and intuitive explanation 
    

%We propose genetic algorithm  based framework for producing adversarial audio samples for a given input is shown in Algorithm~\ref{algo:1}. A genetic algorithm maintains a population of solutions and implements a survival-of-the-fittest strategy in search for the best-fitting solutions. 

 %The remainder of this section relates these stages with the major system components depicted in Fig.~\ref{fig:system} and explains each component in detail\footnote{The code will be open-sourced on acceptance}. 

% \begin{algorithm}[htbp]
% \caption{Framework for producing adversarial audio samples, given an audio input}
% \begin{algorithmic}[1]
% \If {Targeted}
%     \State \textbf{Input:} audio signal: $a$, text: $t=ASR(a)$, \\ target text: $t'', maxiters$ 
% \Else
%     \State \textbf{Input:} audio signal: $a$, text: $t=ASR(a), maxiters$ 
% \EndIf    
% \textbf{Output:}  adversarial audio signal: $a'$ \\
% \end{algorithmic}
% %, adversarial text: $t^{a}=ASR(y^{a})$
% \begin{algorithmic}[1]
% \Procedure{Initialization}{$x$}
% \State $P_{0} \gets [x + w \times \mathcal{N}(\mu,\,\sigma^{2})] * popsize $ \\
% \Return $P_{0}$
% %\Comment{Random Gaussian Noise}
% \EndProcedure \\

% \Procedure{Fitness Computation}{$P$}
% \For {$p \in \mathcal P $}
% \State $t' \gets ASR(p)$
% %\State $FV \gets MFCC(p)$
%  \If {Targeted}
% \State $f_{1} \gets EditDistance(t', t'')$   \Comment{minimized}
% \Else
% \State $f_{1} \gets EditDistance(t', t)$
% \Comment{maximized}
% \EndIf
% \State $f_{2} \gets Similarity(MFCC(p), MFCC(a))$
% \EndFor \\
% \Return $f_{1},f_{2}$
% \EndProcedure \\

% \Procedure{Mating Pool Identification}{$P, F$}
% \State $pool_{1} \gets SameRankSelect(P, F)$
% \State $pool_{2} \gets InvertedRankSelect(P, F)$
% \State $pool_{3} \gets RouletteWheelSelect(P, F)$ \\
% \Return $pool_{1} \cup pool_{2} \cup pool_{3}$ \Comment{list of parent pairs}
% \EndProcedure \\

% \Procedure{Crossover}{$ParentPairs$}
% \For {$p_1, p_2$ in $ParentPairs$}:
% \State  $children_{1} \gets \frac{p_{1}+p_{2}}{2} $ 
% \State  $children_{2} \gets \frac{2 \cdot p_{1}+p_{2}}{3}$
% \State  $children_{3} \gets \frac{p_{1}+2 \cdot p_{2}}{3}$
% \EndFor \\
% \Return $children_{1} \cup children_{2} \cup children_{3}$
% \EndProcedure \\

% \Procedure{Mutation}{$children$}
% \For {$c$ in $children$}:
% \State $children_m \gets [c + prob_m \times \mathcal{N}(\mu,\,\sigma^{2})]$ \\
% %\Comment{Random Gaussian Noise}
% \Return $children_m$
% \EndFor
% \EndProcedure \\

% \Procedure{GetDominations}{$P$}
% \State $P_{new} \gets ComputeDominance(P)$
% \State $P_{new} \gets ReRank(P_{new})$ \\
% \Return $P_{new}$
% \EndProcedure \\

% \Repeat
% \State $P_i \gets Initialization(a)$
% \State $F_i \gets FitnessComputation(P_i)$
% \State $parents_i \gets MatingPoolIdentification(P_i, F_i)$
% \State $children_i \gets Mutation(Crossover(parents_i))$
% \State $P_{i+1} \gets GetDominations(parents_i \cup children_i)$
% \Until{$P_i == P_{i+1}$ or $i > maxiters$} \\
% \State $P_{final} = P_{i} $
% \State $a' \gets P_{final}[0]$ \Comment{highest ranked individual}
% \end{algorithmic}
% \label{algo:1}
% \end{algorithm}

% \subsubsection{Population} In genetic systems, each potential solution is termed as an \textit{Individual}. Each individual's characteristics are determined by it's \textit{Genes}. %Genes can be thought of as analogous to model parameters. 
% The group of individual solutions in a genetic system is called its \textit{Population}. The population iteratively gets fitter over time resulting in more optimal solutions. The population in each iteration is known as a \textit{Generation}\footnote{Henceforth; we use the terms population and generation interchangeably}.
% At the beginning of the first generation, genes of the population are either randomly initialized or initialized according to some heuristics which helps the process to converge quickly.

% \subsubsection{Fitness Computation} In order to gauge the optimality of each individual solution, a \textit{Fitness Function} is defined for the problem at hand. The genes of each individual are plugged into the fitness function to get a \textit{Fitness Score}. 

%In literature, adversarial attacks usually use a fitness function with a single objective. Their approaches select elite individuals from the population based on a single criterion. \cite{Alzantot_bb} use the score of the model and \cite{Rohan_BB} use text similarity. These works have ignored acoustic similarity, which is a strong indicator of the goodness of an individual. An audio sample is considered to be a good adversary, if it sounds very similar to the original sample but generates an entirely different text. Hence the sample generated should have: i) maximum acoustic similarity and minimum text similarity (for un-targeted attacks), or ii) maximum acoustic similarity and maximum text similarity with a target text (for targeted attacks). We achieve this by introducing a fitness function with multiple objectives which tries to strike a balance between acoustic and text similarities. 



% \noindent The second child is created such that $p_1$'s characteristics is dominant in its genes

% \begin{equation}
%     \frac{2 \times p_{1}+p_{2}}{3}
% \end{equation}

% \noindent and the third child's genes are dominated by $p_2$'s characteristics.

% \begin{equation}
%     \frac{ p_{1}+2 \times p_{2}}{3}
% \end{equation}



% \begin{figure}
%     \includegraphics[width=\columnwidth]{images/Pareto.png}
%     \caption{A \textit{Pareto Chart} showing the dominance of individuals in various generations for a random audio sample during an un-targeted attack.}
%     \label{fig:pareto_plot}
% \end{figure}

% \textbf{Dominance evaluation} 

% In our system, after a set of offspring is created, their fitness scores are evaluated in the same way as it was done for their parents. The combined set of parents and children are ranked based on their dominance. The most dominating individuals are carried forward to the next generation, and the others are discarded. Fig. \ref{fig:pareto_plot} shows the edit distance and MFCC distance of individuals over generations. The blue points are the individuals of the final generation. We can observe the formation of a \textit{knee curve}, and the individual closest to the \textit{knee point} is considered to be the best solution.

% \subsection{Implementation Details}
% A set of $100$ individuals are created to form the initial population. They are initialized by adding random uniform noise to the original audio signal with a sampling rate of $16,000$. Therefore, a two-second audio clip will result in individuals having $32,000$ genes. Intuitively, this helps in faster convergence when compared to random initialization. 

% After computing the fitness scores based on acoustic (MFCC) and textual (edit distance) similarities, the population is converted to a list of mating pairs. The extraction of MFCC features is performed using python \textit{librosa} library\footnote{https://github.com/librosa/librosa} with window size of $25ms$ and a stride of $10ms$. It is to be noted that an individual may appear in more than one mating pair. The three crossover operations described previously are applied to each pair to produce three children. Probabilistic mutation is applied to every gene of every individual with $prob_m = 0.005$.

% Next, the parents and children are combined and re-ranked based on their dominance and the top $30$ Pareto-optimal individuals are propagated to the next generation. This process is repeated for a $maxiters = 50$, or until we get the same set of Pareto-optimal solutions over two successive generations which indicates convergence. The most dominant individual from the last generation is the adversarial counterpart for our input audio signal. After termination, there may be multiple, equally good dominant solutions to pick from (with equal dominance). In this case, we choose one at random as the best solution.
% \begin{figure}[t]
%      \centering
%      \includegraphics[width=\columnwidth]{images/waveform.png}
%     \caption{Overlay of an original sample (text: "i've got to go to him") on an adversarial sample (text: "it got girl") shown in the time domain.}
%  \label{fig:overlay}
%  \end{figure}
%We run all the experiments on a $16$ core machine with $64$GB of RAM. A typical two-second clip will converge in $\sim60$ minutes showcasing the speed of our approach.

% The fitness of each member is determined using text similarity quantify by edit distance\cite{} and the acoustic similarity is determined by Mel frequency cepstral coefficients(MFCC)\cite{}.  MFCC are robust features that approximate the human auditory system. The derivatives capture the temporal evolution of the audio signal. MFCCs are a traditional feature used for the tasks like audio retrieval, automatic speech recognition, etc. for the representation of an audio signal. MFCC takes human perception sensitivity with respect to frequencies into consideration and hence have been used for the task. The acoustic similarity is a function of the Euclidean distance between MFCC features of the two audio samples. 

% For un-targeted attacks on the ASR system, the ideal candidate is the one having minimum Euclidean distance (maximum acoustic similarity) and maximum Edit distance. Whereas for the targeted attacks where we expect the ASR to generate a particular text for the given sample the best candidate should have minimum edit distance and minimum (maximum acoustic similarity) 

% Further, mutation operation is performed to change the genetic information. Mutation is needed because even though reproduction and crossover effectively recombine existing information, occasionally some useful genetic information might be lost. The mutation operation protects against such irrecoverable loss. It also introduces additional diversity into the population. 

% The gene representing the audio signal is mutated with a probability $p \in0.005 \sim 1 $ ,by adding random noise sampled from a uniform distribution by generating a random number $0<r<1$, if $r<p$. For all the offsprings, we compute the fitness and rank the offsprings. As discussed earlier, the key concept of multi-objective optimization is dominance. Rank is defined as the number of members that dominate it plus one. In multi-objective optimization, the rank is crucial in determining which population member are the fittest. A solution of rank one is said to be Pareto optimal, and the set of rank one points for a given generation is called the Pareto set. As the number of generations increases and the fitness of the population improves, the size of the Pareto set grows.

% Based on these ranks, we conduct the tournament and replace parent population by the better members of the combined population. This process is done for maximum iteration or until convergence is reached, the convergence is checked once the members of Pareto set do not change.  The adversarial solution is identified as the best rank solution in the pareto set. 

% This is much better than using composite weighted functions in conjunction with gradient-based methods since there is no need to solve the problem for various weights. The concept of dominance performs a natural selection of the best adversarial audio sample to fool an  ASR system. It is essential for an adversarial sample to sound exactly similar to the original signal, however, the text produced is extremely different.  Our proposed algorithm employs multi-objective optimization to perform this task.    

% \begin{figure}
%     \centering
%     \includegraphics{pareto-front.png}
%     \caption{Pareto Front }
%     \label{fig:my_label}
% \end{figure}{}
% \end{document}



==> literature.tex <==
\section{Existing Literature}

% Should have  papers characterized as : 
% \begin{enumerate}
%     \item Work in image domain 
%     \item White box attacks in speech domain
%     \item Black box attacks in speech domain 
%             Genetics Algorithms 
%             drawback of the two paper: (Alzantot,Rohan Atori)
% \end{enumerate}

\subsection{Adversarial Generation in Vision} 
\cite{Goodfellow} demonstrated that neural networks are vulnerable to very small changes in the input. These changes, which are indistinguishable to the human eye, cause the classifier to mis-classify the input. They developed the Fast Gradient Sign Method (FGSM) for generating adversarial examples to showcase that the state-of-the-art neural models are not robust to minute adversarial perturbations introduced in their inputs. This work triggered a huge interest in the community and various approaches have been proposed for increasing the robustness of networks for tasks like image classification, face detection, image segmentation, etc. \cite{PapernotMGJCS16,Szegedy,adv_imag,2017arXiv170206832K,2017arXiv171109856A}. 
%text classification and malware detection   

%\textbf{ below para can be part of intro also white box setting or black box setting targetted and untargetted}
%Based on the information available to the attacker,  the neural network system can be deceived in two ways: black box attacks and white box attacks.  In white box attacks, the attacker is conscious of the internals of the network, it weights, gradients etc. whereas in a black box setting he is aware only of the output put of the system and no internal knowledge about the components of the network.    Additionally,  the intent of the attacker can be to construct a sample ${X}'$ for a given input $X$, such that $Model(x)  \neq  Model ({X}')$. Such intents are termed as Un-targetted  attacks.  Where the intent of the attacker is to generate an specific sample ${X}'$ where  besides the output of the model for both the inputs must differ, it should be assigned with a specific label. 

%White box attacks have been mostly successful using techniques like FGSM or DeepFool 

\subsection{Adversarial Generation in Audio} 
In contrast to images, audio presents additional challenges for attackers to deal with.  Majority of image-based deep learning models directly operate at the pixel level. However, ASR attacks require the input to be pre-processed to some intermediate representation. For example, an audio waveform is usually transformed by: i) obtaining the Mel-frequency Cepstrum Coefficients (MFCC) as features, or ii) transformed in the frequency domain to obtain a spectrogram, which is then fed into ASR systems. \cite{Ciss2017HoudiniFD} proposed a framework which can be used to attack a variety of deep learning models, both for image and audio inputs. But the framework was only able to generate the adversarial spectrogram for audio samples and not the actual audio samples themselves. Rebuilding time domain signals from a spectrogram is difficult due to overlapping windows  which are used for analysis. This makes adjacent components in a spectrogram dependent on each other.  

In ~\cite{Iter2017GeneratingAE}, the proposed approach generated adversarial speech samples for ASR systems by adding perturbations to the MFCC features and performing lossy reconstruction of the speech signal in the time domain. This lossy reconstruction made the perturbations perceptible to the human ear. ~\cite{carlini} developed a method which enabled the propagation of gradients to the MFCC reconstruction layer. They performed white box targeted attacks on Mozilla's Deepspeech\footnote{\url{https://github.com/mozilla/DeepSpeech}} model and obtained adversarial samples which were $99.9\%$ similar to the desired target text.   

Furthermore, works like~\cite{backdoor,dolphinattack} have utilized non-linearities of microphones in smart devices to generate commands (adversarial examples with frequency $~40$Khz.) audible only to speech assistants and not to humans. Another kind of attack proposed in ~\cite{hiddenvoicecommands} intends to generate sounds that are interpreted as voice commands by devices but are unrecognizable to human listeners. These attacks, although powerful, are usually easy to detect or prevent.

%In real - life scenarios, it is impractical to assume access to underlying details of ASR like models gradients and architecture.  Hence to test the robustness of the ASR systems adversarial samples generated using black box approach play a more important role.  

%This paper’s adopts black box approach to adversarial sample generation.  It uses a combination of genetic algorithm and gradient estimation for the task.  Their approach is an extension of work done by Alzantot which works on single words(speech commands). 
\subsection{Adversarial Generation in Audio with Genetic Algorithms}
%As mentioned in the work by \cite{Alzantot_bb,Rohan_BB}, targetted black box attacks have been performed on ASR using genetic algorithms. 
\cite{Alzantot_bb} used a genetic algorithm to perform a black-box attack on audio samples containing short speech commands. Each waveform belonged to a pre-defined class and the attack changed the way they were classified. This was done by iteratively applying noise to the audio samples. 

\cite{Rohan_BB} extended this approach to work on longer phrases and sentences. Their approach is limited to ASR systems which give access to the last layer (logits) of the model and hence is limited to systems like Mozilla  Deepspeech.  Additionally, their approach can be considered as \textit{Grey-box} at best, as the attacks are generated based on prior knowledge of the model's loss function and may not scale to other ASRs. These works perform targeted attacks using a genetic algorithm by minimizing the some distance metric between the actual text and the text generated by the ASR with the adversarial audio as input and do not use any features to capture acoustic similarity between the adversarial sample and original sample.   

In our work, we consider adversarial audio generation as a multi-objective optimization problem which should  achieve a balance between conflicting objectives. As far as we know, we are the first to propose, implement and evaluate such a framework for adversarial audio generation. 

% % Targeted Adversarial Examples for Black Box Audio Systems  (Submitted To NIPS) [Rohan Atori]
% The paper identifies an important problem of black box testing of speech recognition system. However, this work lacks  experimentation to prove their results in the following aspects: 
% 1. Since the authors claim that their approach is black box , experiments should include testing of few more end to end speech recognition system. 
%     1. The approach proposed by authors seems to extremely coupled with techniques used in deep speech model , hence it might only work for that. 
%     2. The sample provided by the authors, and few generated using the code base don’t act as adversarial for speech to text system like: 
%         1. Google speech to text api (https://cloud.google.com/speech-to-text/)
%         2. IBM speech to text api (https://speech-to-text-demo.ng.bluemix.net/)
%         3. Adversarial samples tried: 
% 			1. “He wasn't asking for help”
% 			2. “And you know it” 
% 			3. “I’ve got to go to him.”
% 			4. “I make my living forecasting the future for people to set.”
% 		Few more samples were generated but these didn’t act as adversarial samples for the above two ASR system.
% 2.	Qualitative evaluation of adversarial samples generated should be performed to understand how similar it is to the actual audio for human ear.

% Lack of experimentation makes it  difficult to comprehend the robustness of their approach. 


%DolphinAttack [13] exploits the same non-linearities in microphones to create commands audible to speech assistants but inaudible to humans. Notably, in both methods [11, 13] the attack sound is not heard by the human at all, while an adversarial example should be recognized by a human as benign while misclassified by the speech recognition model.


%Therefore using floating point numbers to represent the variables in most problems is more logical which requires less storage than binary coded strings.  --- Alzantot use binary encoding (confirm again)

